Can Language Model Understand Word Semantics as A Chatbot? An Empirical Study of Language Model Internal External Mismatch

Current common interactions with language models is through full inference. This approach may not necessarily align with the model's internal knowledge. Studies show discrepancies between prompts and internal representations. Most focus on sentence understanding. We study the discrepancy of word semantics understanding in internal and external mismatch across Encoder-only, Decoder-only, and Encoder-Decoder pre-trained language models.

==> intro.tex <==
\section{Introduction}

Language models (LMs)~\citep{bert,radford2019language,gpt-j,gpt3} have drawn a wide range of interest in many fields.
The ability to process natural language, encode data into parameters, and generate convincing paragraphs drive many people to consider it as trusted knowledge source.
LM's truthfulness is then a key factor to determine if they are suitable for many downstream applications;
in other word, researchers need to assess LMs integrity in their claims.

The foundation of transformer-based LMs is a next token generator, $P(token|input)$.
Prompt engineering \xyz{ref cot?} demonstrates a significant improvement of LM's reasoning performance and 
it promotes interaction with models in a end-to-end inference manner.
Focusing on the inference, 
many research groups reveal that LMs shows poor performance in semantic understanding and linguistic cognition
\xyz{ref Dentella et al. (2023), Katzir (2023)}.

Thus, researchers must delve deeper into the correlations right before generating the very next token 
\xyz{refs here about logits study}. 
Before sampling a token with common strategy like top-K,
we can access the probability of vocabulary, known as logits.
Examining logits depicts the confidence of the model to generate the next token.
For example, when the input prompt is a yes-no question,
comparing the probility between token \textit{Yes} and \textit{No} would describe the model's choice as well as the confidence level of the model. 

Understanding the semantics of a word in the context of sentences falls into natrual language processing (NLP).
Since the introduction of BERT \xyz{ref here},
transformer-based models show exceptional performance,
especially in understanding the contextual meaning of words.
However, we show that the discrepancy between the LM's external response and its internal representation hinders LM's performance.
This mismatch impacts the trustworthiness of context generated by LMs,
which may cause further harms when people regard the LM's generation as a knowledge source. 
\xyz{ref (Ji et al., 2023).}

This work mainly focus on the truthfulness of LMs in word semantics.
We find that even if the LM's output is incorrect,
it is possible for the internal representation to disagree.
To study the mismatch, 
we adopt two ways of interaction with the LMs:
\textcircled{\small 1}
\textbf{querying} is to directly ask the auto-regressive, generative model for an output;
\textcircled{\small 2}
\textbf{probing} occurs when we extract the last hidden state information during the generation phase and then train the probe for classification.
For example, give a question prompt for BERT,
\begin{framed}
% \noindent\textit{\{Sentence1\}\\\{Sentence2\}\\ Does the word "\{word\}" mean the same thing in the above two sentences?\\
\noindent
"A keen musical sense ."\\
"A good sense of timing ."\\
Does the word "sense" mean the same in the above two sentences?\\
Answer:[MASK]
\end{framed}
% \begin{tabular}{p{0.8\linewidth}}
% "A keen musical sense ."\\
% "A good sense of timing ."\\
% Does the word "sense" mean the same in the above two sentences?\\
% Answer:[MASK]
% \end{tabular}
\noindent
BERT fills the masked token with a \textit{Yes},
and the process is known as querying.
Right before BERT decodes the output of the transformer layers to logits, 
we perform probing to collect the internal representations, which is also known as the last hidden state.
The collected internal representations are then used to train a binary classifier as per \xyz{ref Reimers and G} and apply it to the test / validation set for correctness.

Surprisingly, the embedding probing shows consistent higher accuracy in comprehending the word semantics.
The observation could be that LMs understand the word semantics but somehow ignored this knowledge when decoding the last hidden state to logits. 
Understanding the word semantics goes beyond the linear probing in real-world applications;
additionally probing is not completely better on each individual questions.
Decoding the last hidden state into logits should catch up the probing performance;
it could be a sign that further alignment or calibration on models is necessary.



one of their most prominent drawbacks is generating inaccurate or false information with a confident tone

Figure~\ref{fig:cute} depicts

\begin{figure*}[htb!]
\includegraphics[width=\linewidth]{./figures/cute.png}
\caption{The discrepancy between internal representations of the word semantics and external expressions of similarity probability. Querying is the end-to-end inference; probing is the trained classifier.}
\label{fig:cute}
\end{figure*}

% \newpage
\section{Related Works}

\paragraph{Model Honesty}  This work is related to honesty~\citep{honesty}. Honesty intersects with aspects such as truthfulness~\citep{evans2021truthful}, calibration~\citep{guo2017calibration,calirevisit,10.1162/tacl_a_00494}, self-knowledge~\citep{llmknwodk,llmknow}, non-deceptiveness~\citep{internallie} and so on. 
There are works investigating whether AI models are aware of what they are expressing. 
The comprehensive analysis on the honesty of LLMs by ~\citet{llmknow} concludes that LLMs are well-calibrated.~\citet{cheng2024can} has similar conclusions regarding models' awareness and understanding of what they know and what they do not know. Other works also demonstrated quirky behaviors and phenomena associated with how the model respond to prompt~\citep{khashabi-etal-2022-prompt,webson-etal-2023-language}. 

The most relevant research to ours are ~\citet{prompt-prob}, ~\citet{probing-query} and ~\cite{internallie}. ~\citet{prompt-prob} explored the discrepancies between the model's internal next token distribution and the distribution obtained using prompts such as \textit{"What is the best next word?"}.
~\citet{probing-query} analyzed the internal and external inconsistencies of the model from the perspectives of probing(internal) and querying(external). ~\citet{internallie} investigated how to use the internal state to determine the truthfulness of text generated by language models, thereby also confirming inconsistencies between the model's internal and external outputs. Our work investigates the semantics of word inconsistencies between internal states and prompts.

\paragraph{Word Embeddings} Word2vec~\citep{word2vec} first uses dense vector representations to represent words. Subsequently, GloVe~\cite{glove} enhanced this concept by considering word co-occurrence within the text, offering richer representations. Despite their efficacy, these models including~\citep{fasttext,LexVec,PTE} provide static embeddings, where each word has a fixed representation regardless of the context. 
ELMo~\citep{elmo} is the first to introduced the concept of contextual embeddings by adapting embeddings to word usage in context. 
BERT~\citep{bert} utilizes transformer architecture to capture deep contextual nuances, setting new standards for various NLP tasks. 
Building on this, GPT~\citep{gpt3}, RoBERTa~\citep{liu2019roberta}, XLNet~\citep{yang2019xlnet}, and Transformer-XL~\citep{transformerxl}, each introduced innovations that refined and expanded the capabilities of NLP models, moving towards a better context-aware language understanding.

In the case of contextual word embeddings, the approach extends beyond merely leveraging the embedding layer; researchers incorporate the hidden layers as well. Some research~\citep{yang2019xlnet} opts to use the last hidden layer as the source of embeddings for downstream applications. Alternatively, a concatenation of all hidden layers is employed by others to enrich the embeddings~\citep{elmo}. In our work, we have chosen to utilize the last hidden layer as our word embedding.


==> tbl/main_result.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{cc|c|ccc|c}
\hline
    Model    &  method     & WiC  & \multicolumn{3}{c|}{NER}  & CoLLN2003 \\ \hline
        &       &  Acc(\%)    & precision & recall & F1  & Acc(\%)     \\ \hline
BERT-base    & Query & 50 & 7 & 100 & 14& 25   \\
        & Prob & 65 & 95 & 96 & 96& 51     \\   \hline
BERT-large    & Query & 53 & 3 & 100 & 6& 26   \\
        & Probe & 65 &  96& 95 &96 & 48    \\ \hline
GPT2    & Query & 49 & 4& 42 & 8& 33    \\
        & Probe & 58 &97& 32& 48& 41    \\ \hline        
T5-small& Query & 49 & 5 & 8& 6& 31    \\
        & Probe & 61 & 98& 94& 96& 47    \\ \hline
T5-large& Query & 50 & 5 & 8& 6& 31    \\
        & Probe & 65 & 98& 94& 96& 47    \\ \hline
% Flan-T5 & query & 0.51 &      &         \\
%         & probe & 0.60 &      &        \\ \hline
\end{tabular}
\caption{Accuracy of representative encoder, decoder, and encoder-decoder models on benchmark WIC, NER, and Analogy.}
\label{tbl:main}
\end{table*}
